A survey of uncertainty principles and some signal processing applications

The goal of this paper is to review the main trends in the domain of uncertainty principles and localization, emphasize their mutual connections and investigate practical consequences. The discussion is strongly oriented towards, and motivated by signal processing problems, from which significant advances have been made recently. Relations with sparse approximation and coding problems are emphasized.

==> mydefs.tex <==
\def\matlab{{\sc Matlab\ }}
\def\octave{{\sc Octave}}


\def\foorp{{\hfill$\spadesuit$}}
\def\ds{{\displaystyle}}
\def\inv{{^{-1}}}
\def\HH{{\mathbb H}}
\def\MM{{\mathbb M}}
\def\tMM{\tilde{\mathbb M}}
\def\RR{{\mathbb R}}
\def\PP{{\mathbb P}}
\def\EE{{\mathbb E}}
\def\Pr#1{{\PP\!\left\{#1\right\}}}
\def\Ex#1{{\EE\left\{#1\right\}}}
\def\var#1{{\hbox{Var}\left\{#1\right\}}}
\def\QQ{\mathbb Q}
\def\CC{\mathbb C}
\def\ZZ{\mathbb Z}
\def\NN{\mathbb N}
\def\Id{{\mathbbm 1}}

\def\tX{\tilde{X}}

\def\o{\overline}
\def\la{\langle}
\def\ra{\rangle}

\def\ch{{\rm ch}}
\def\sh{{\rm sh}}


\def\rf#1{(\ref{#1})}
\def\be{\begin{equation}}
\def\beq#1{\begin{equation}\label{#1}}
\def\ee{\end{equation}}
\def\bea{\begin{eqnarray}}
\def\beqa#1{\begin{eqnarray}\label{#1}}
\def\eea{\end{eqnarray}}
\def\ba{\begin{array}}
\def\ea{\end{array}}


\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}


\def\cA{{\mathcal A}}
\def\cB{{\mathcal B}}
\def\cC{{\mathcal C}}
\def\tcC{\tilde{\mathcal C}}
\def\cD{{\mathcal D}}
\def\cE{{\mathcal E}}
\def\cF{{\mathcal F}}
\def\ocF{\overline{\mathcal F}}
\def\cH{{\mathcal H}}
\def\ck{{\mathcal k}}
\def\cK{{\mathcal K}}
\def\cL{{\mathcal L}}
\def\cM{{\mathcal M}}
\def\cN{{\mathcal N}}
\def\cP{{\mathcal P}}
\def\cR{{\mathcal R}}
\def\cS{{\mathcal S}}
\def\cU{{\mathcal U}}
\def\cV{{\mathcal V}}
\def\cW{{\mathcal W}}
\def\cl{{\mathpzc l}}
\def\cs{{\mathpzc s}}




\def\la{{\langle}}
\def\ra{{\rangle}}
\def\qed{\hskip 6pt\vrule height6pt width5pt depth1pt}
\def\R{\RR}
\def\Z{\ZZ}
\def\sgn{\hbox{sgn}}
\def\Lone{L^1(\RR )}
\def\Ltwo{L^2(\RR )}
\def\Linf{L^\infty(\RR )}
\def\Lba{L^2(\RR\times\RR_+^* ,a^{-1}dadb)}
\def\Htwo{H^2(\RR )}
\def\lone{\ell^1(\ZZ )}
\def\ltwo{\ell^2(\ZZ )}
\def\gets{$<\!\!\! -\,$}
%\def\Id{{\bf 1}}
\def\bds{_{-\infty}^\infty}
\def\supp{\hbox{supp}}
\def\mod{{\mathrm {mod}}}
\def\modN{[\hbox{\footnotesize mod }N]}

% bold
\def\bm{{\mathbf m}}
\def\bG{{\mathbf G}}
\def\br{{\mathbf r}}
\def\bu{{\mathbf u}}
\def\bU{{\mathbf U}}
\def\bv{{\mathbf v}}
\def\bV{{\mathbf V}}
\def\bx{{\mathbf x}}
\def\by{{\mathbf y}}
\def\bY{{\mathbf Y}}
\def\bpsi{\boldsymbol{\psi}}
\def\bPsi{\boldsymbol{\Psi}}
\def\bg{{\mathbf g}}
\def\bS{{\mathbf S}}
\def\bh{{\mathbf h}}
\def\balpha{\boldsymbol{\alpha}}
\def\ba{{\mathbf a}}
\def\bzero{\boldsymbol{0}}
\def\bT{{\mathbf T}}
\def\blambda{\boldsymbol{\lambda}}
\def\bw{{\mathbf w}}
\def\bM{{\mathbf M}}
\def\bB{{\mathbf B}}
\def\bq{{\mathbf q}}
\def\bb{{\mathbf b}}
\def\bI{{\mathbf I}}
\def\bO{{\mathbf 0}}

% overline
\def\ox{\overline{x}}
\def\oy{\overline{y}}
\def\oz{\overline{z}}

% tilde
\def\tb{{\tilde{b}}}
\def\te{{\tilde{e}}}
\def\tf{{\tilde{f}}}
\def\tg{{\tilde{g}}}
\def\th{{\tilde{h}}}
\def\tk{{\tilde{k}}}
%\def\tt{{\tilde{t}}}
\def\tp{{\tilde{p}}}
\def\tu{{\tilde{u}}}
\def\tv{{\tilde{v}}}
\def\tx{{\tilde{x}}}
\def\ty{{\tilde{y}}}
\def\tz{{\tilde{z}}}
\def\tp{{\tilde{p}}}
\def\tq{{\tilde{q}}}

\def\tgamma{{\tilde\gamma}}
\def\tGamma{{\tilde\Gamma}}
\def\tsigma{{\tilde\sigma}}
\def\tSigma{{\tilde\Sigma}}
\def\tpi{{\tilde\pi}}
\def\tpsi{{\tilde\psi}}
\def\trho{{\tilde\rho}}
\def\tX{{\tilde{X}}}
\def\tY{{\tilde{Y}}}
\def\S{{\tilde{S}}}
\def\T{{\tilde{T}}}

% hat
\def\hb{{\hat b}}
\def\he{{\hat e}}
\def\hh{{\hat h}}
\def\hk{{\hat k}}
\def\hp{{\hat p}}
% \def\ht{{\hat t}}
\def\hu{{\hat u}}
\def\hv{{\hat v}}
\def\hw{{\hat w}}
\def\hx{{\hat x}}
\def\hy{{\hat y}}
\def\hz{{\hat z}}
\def\hLambda{{\hat \Lambda}}
\def\hDelta{{\hat \delta}}
\def\hlambda{{\hat \lambda}}
\def\hdelta{{\hat \delta}}
\def\halpha{{\hat \alpha}}
\def\hbeta{{\hat \beta}}
\def\htheta{{\hat \theta}}
\def\hsigma{{\hat \sigma}}


% vectors (underline)
\def\a{{\underline{a}}}
\def\b{{\underline{b}}}
\def\e{{\underline{e}}}
\def\h{{\underline{h}}}
\def\k{{\underline{k}}}
\def\m{{\underline{m}}}
\def\t{{\underline{t}}}
\def\u{{\underline{u}}}
\def\v{{\underline{v}}}
\def\w{{\underline{w}}}
\def\x{{\underline{x}}}
\def\y{{\underline{y}}}
\def\z{{\underline{z}}}

\def\X{{\underline{X}}}
\def\Y{{\underline{Y}}}
\def\S{{\underline{S}}}
\def\T{{\underline{T}}}

\def\Om{{\underline{\Omega}}}

\def\ual{{\underline\alpha}}
\def\ubet{{\underline\beta}}
%
% Matrices
\def\A{{\underline{\underline{A}}}}
\def\RX{{\underline{\underline{R}}_X}}

%
% Algebraic quantities
\def\rg#1{{\hbox{rg}\left(#1\right)}}

